Data-Driven Learning of Geometric Scattering Networks

We propose a new graph neural network (GNN) module, based on relaxations of recently proposed geometric scattering transforms, which consist of a cascade of graph wavelet filters. Our learnable geometric scattering (LEGS) module enables adaptive tuning of the wavelets to encourage band-pass features to emerge in learned representations. The incorporation of our LEGS-module in GNNs enables the learning of longer-range graph relations compared to many popular GNNs, which often rely on encoding graph structure via smoothness or similarity between neighbors. Further, its wavelet priors result in simplified architectures with significantly fewer learned parameters compared to competing GNNs. We demonstrate the predictive performance of LEGS-based networks on graph classification benchmarks, as well as the descriptive quality of their learned features in biochemical graph data exploration tasks.

==> tables/biochem_comparison.tex <==
\begin{table*}[tb]
    \caption{Mean $\pm$ standard deviation test set accuracy on biochemical datasets. TLE denotes models that exceeded the 10 hour time limit.}
    \begin{center}
    \begin{small}
    \begin{sc}
    \vskip 0.1in
    \scalebox{0.95}{
        \input{tables/raw/biochen_comparison_raw}
    }
    \label{tab:bio_comp}
    \end{sc}
    \end{small}
    \end{center}
    \vskip -0.1in
\end{table*}


==> tables/biochem_stats.tex <==
%\begin{wraptable}[11]{r}{0.7\textwidth}
%\vspace{-12pt}
\begin{table}[ht]
    \centering
\caption{Dataset statistics, diameter, nodes, edges, and clustering coefficient averaged over graphs.}
 \label{tab:biochem_stats}
%\vspace{-3pt}
\adjustbox{width=\linewidth}{
    \begin{tabular}{lrrrrrr}
\toprule
{} &  \# Graphs &  \# Classes &  Diameter &   Nodes &    Edges &  Clust. Coeff \\
\midrule
DD               &      1178 &          2 &     19.81 &  284.32 &   715.66 &          0.48 \\
ENZYMES          &       600 &          6 &     10.92 &   32.63 &    62.14 &          0.45 \\
MUTAG            &       188 &          2 &      8.22 &   17.93 &    19.79 &          0.00 \\
NCI1             &      4110 &          2 &     13.33 &   29.87 &    32.30 &          0.00 \\
NCI109           &      4127 &          2 &     13.14 &   29.68 &    32.13 &          0.00 \\
PROTEINS         &      1113 &          2 &     11.62 &   39.06 &    72.82 &          0.51 \\
PTC              &       344 &          2 &      7.52 &   14.29 &    14.69 &          0.01 \\
\bottomrule
\end{tabular}
}
\end{table}


==> tables/casp_by_target.tex <==
\begin{table}[!t]
    \centering
     \caption{Test set mean squared error on CASP GDT regression task across targets over 3 non-overlapping test sets.}
    \scalebox{0.7}{
\begin{tabular}{llllllll}
\toprule
{} &                     LEGS-RBF &                     LEGS-FCN &                   LEGS-FIXED &                 GCN &           GraphSAGE &              GIN                &            Baseline \\
\midrule
t0860 &           197.68 $\pm$ 34.29 &  \textbf{164.22 $\pm$ 10.28} &           206.20 $\pm$ 28.46 &  314.90 $\pm$ 29.66 &  230.45 $\pm$ 79.72 &           262.35 $\pm$ 66.88 &  414.41 $\pm$ 26.96 \\
t0868 &            131.42 $\pm$ 8.12 &  \textbf{127.71 $\pm$ 14.26} &            178.45 $\pm$ 5.64 &  272.14 $\pm$ 26.34 &  191.08 $\pm$ 21.96 &           170.05 $\pm$ 27.26 &  411.98 $\pm$ 57.39 \\
t0869 &            106.69 $\pm$ 9.97 &           132.12 $\pm$ 31.37 &  \textbf{104.47 $\pm$ 14.16} &  317.22 $\pm$ 12.75 &  244.38 $\pm$ 40.58 &           217.02 $\pm$ 57.01 &  393.12 $\pm$ 48.70 \\
t0872 &           144.11 $\pm$ 24.88 &           148.20 $\pm$ 23.63 &   \textbf{134.48 $\pm$ 8.25} &  293.96 $\pm$ 19.00 &  221.13 $\pm$ 28.74 &           240.89 $\pm$ 24.17 &  374.48 $\pm$ 33.70 \\
t0879 &            89.00 $\pm$ 44.94 &            80.14 $\pm$ 16.21 &   \textbf{64.63 $\pm$ 15.92} &  309.23 $\pm$ 69.40 &  172.41 $\pm$ 73.07 &           147.77 $\pm$ 15.72 & 364.79 $\pm$ 144.32 \\
t0900 &           193.74 $\pm$ 10.78 &           171.05 $\pm$ 25.41 &   \textbf{158.56 $\pm$ 9.87} &  254.11 $\pm$ 18.63 &  209.07 $\pm$ 11.90 &           265.77 $\pm$ 79.99 &  399.16 $\pm$ 83.48 \\
t0912 &  \textbf{113.00 $\pm$ 22.31} &           169.55 $\pm$ 27.35 &            150.70 $\pm$ 8.53 &  227.17 $\pm$ 22.11 &  192.28 $\pm$ 39.45 &           271.30 $\pm$ 28.89 &  406.25 $\pm$ 31.42 \\
t0920 &   \textbf{80.46 $\pm$ 14.98} &           136.94 $\pm$ 36.43 &            84.83 $\pm$ 19.70 &  361.19 $\pm$ 71.25 &  261.72 $\pm$ 59.67 &           191.86 $\pm$ 37.85 &  398.22 $\pm$ 25.60 \\
t0921 &           187.89 $\pm$ 46.15 &           165.97 $\pm$ 42.39 &  \textbf{142.97 $\pm$ 27.09} &  382.69 $\pm$ 20.27 &  260.49 $\pm$ 16.09 &           207.19 $\pm$ 24.84 &  363.92 $\pm$ 35.79 \\
t0922 &           254.83 $\pm$ 91.28 &  \textbf{110.54 $\pm$ 43.99} &           227.73 $\pm$ 26.41 &   366.72 $\pm$ 8.10 &   290.71 $\pm$ 7.22 &           130.46 $\pm$ 11.64 &  419.14 $\pm$ 45.49 \\
t0942 &           188.55 $\pm$ 11.10 &           167.53 $\pm$ 22.01 &   \textbf{137.21 $\pm$ 7.43} &   371.31 $\pm$ 9.90 &  233.78 $\pm$ 84.95 &           254.38 $\pm$ 47.21 &  393.03 $\pm$ 24.93 \\
t0944 &            146.59 $\pm$ 8.41 &  \textbf{138.67 $\pm$ 50.36} &           245.79 $\pm$ 58.16 &   263.03 $\pm$ 9.43 &  199.40 $\pm$ 51.11 &            157.90 $\pm$ 2.57 &  404.12 $\pm$ 40.82 \\
\bottomrule
\end{tabular}
}
   
    \label{tab:casp_by_target}
\end{table}


==> tables/chorddiagram-gcn.tex <==
\begin{table}[ht]
    \centering
     \caption{ENZYME Class Preferences Inferred from a GCN mean-pooling graph embedding. The self-affinities have been removed. }
\begin{tabular}{lrrrrrr}
\toprule
{} &  Class 1 &  Class 2 &  Class 3 &  Class 4 &  Class 5 &  Class 6 \\
\midrule
Class 1 &    0.000 &    0.037 &    0.033 &    0.039 &    0.032 &    0.034 \\
Class 2 &    0.033 &    0.000 &    0.029 &    0.033 &    0.028 &    0.030 \\
Class 3 &    0.033 &    0.032 &    0.000 &    0.037 &    0.034 &    0.035 \\
Class 4 &    0.053 &    0.051 &    0.050 &    0.000 &    0.051 &    0.055 \\
Class 5 &    0.027 &    0.026 &    0.029 &    0.031 &    0.000 &    0.021 \\
Class 6 &    0.021 &    0.021 &    0.022 &    0.025 &    0.016 &    0.000 \\
\bottomrule
\end{tabular}

   
\end{table}

==> tables/chorddiagram-plain.tex <==
\begin{table}[ht]
    \centering
    \caption{ENZYME Class Preferences Inferred from LEGS-FIXED. The self-affinities have been removed. }
\begin{tabular}{lrrrrrr}
\toprule
{} &  Class 1 &  Class 2 &  Class 3 &  Class 4 &  Class 5 &  Class 6 \\
\midrule
Class 1 &    0.000 &    0.026 &    0.023 &    0.024 &    0.024 &    0.023 \\
Class 2 &    0.074 &    0.000 &    0.071 &    0.069 &    0.067 &    0.069 \\
Class 3 &    0.031 &    0.034 &    0.000 &    0.032 &    0.031 &    0.031 \\
Class 4 &    0.038 &    0.039 &    0.037 &    0.000 &    0.037 &    0.038 \\
Class 5 &    0.021 &    0.020 &    0.019 &    0.020 &    0.000 &    0.019 \\
Class 6 &    0.017 &    0.018 &    0.017 &    0.017 &    0.016 &    0.000 \\
\bottomrule
\end{tabular} % :) 

    
\end{table}

==> tables/chorddiagram-sort.tex <==
\begin{table}[ht]
    \centering
      \caption{ENZYME Class Preferences Inferred from LEGS-FCN. The self-affinities have been removed. }
\begin{tabular}{lrrrrrr}
\toprule
{} &  Class 1 &  Class 2 &  Class 3 &  Class 4 &  Class 5 &  Class 6 \\
\midrule
Class 1 &    0.000 &    0.029 &    0.027 &    0.027 &    0.025 &    0.025 \\
Class 2 &    0.048 &    0.000 &    0.044 &    0.043 &    0.048 &    0.048 \\
Class 3 &    0.032 &    0.033 &    0.000 &    0.031 &    0.031 &    0.031 \\
Class 4 &    0.036 &    0.036 &    0.035 &    0.000 &    0.036 &    0.035 \\
Class 5 &    0.030 &    0.035 &    0.031 &    0.032 &    0.000 &    0.031 \\
Class 6 &    0.027 &    0.031 &    0.028 &    0.028 &    0.028 &    0.000 \\
\bottomrule
\end{tabular}


  
\end{table}

==> tables/chorddiagram-true.tex <==
\begin{table}[ht]
    \centering
    \caption{ENZYME Class Preferences observed by \cite{cuesta_classification_2015}. The self-affinities have been removed, and the values have been normalized by matrix sum.}
\begin{tabular}{lrrrrrr}
\toprule
{} &  Class 1 &  Class 2 &  Class 3 &  Class 4 &  Class 5 &  Class 6 \\
\midrule
Class 1 &    0.000 &    0.060 &    0.025 &    0.037 &    0.019 &    0.016 \\
Class 2 &    0.060 &    0.000 &    0.092 &    0.108 &    0.024 &    0.027 \\
Class 3 &    0.025 &    0.092 &    0.000 &    0.025 &    0.010 &    0.013 \\
Class 4 &    0.037 &    0.108 &    0.025 &    0.000 &    0.025 &    0.009 \\
Class 5 &    0.019 &    0.024 &    0.010 &    0.025 &    0.000 &    0.011 \\
Class 6 &    0.016 &    0.027 &    0.013 &    0.009 &    0.011 &    0.000 \\
\bottomrule
\end{tabular}

    
\end{table}

==> tables/class-exchange-quantified.tex <==
\begin{table}[t]
\begin{center}
\begin{small}
\begin{sc}
\caption{Quantified distance between the empirically observed enzyme class exchange preferences of \cite{cuesta_classification_2015} and the class exchange preferences inferred from LEGS-FIXED, LEGS-FCN, and a GCN. We measure the cosine distance between the graphs represented by the chord diagrams in Figure~\ref{fig:ribbon}. As before, the self-affinities were discarded. LEGS-Fixed reproduces the exchange preferences the best, but LEGS-FCN still reproduces well and has significantly better classification accuracy.}
\label{tab:equant}
\begin{tabular}{rrr}
\toprule
 LEGS-FIXED &   LEGS-FCN &  GCN\\
\midrule
0.132 &  0.146 &  0.155\\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\end{table}

==> tables/dataset_stats.tex <==
\begin{table}[ht]
    \caption{Dataset statistics, diameter, nodes, edges, clustering coefficient (CC) averaged over all graphs. Split into bio-chemical and social network types.}\label{tab:dataset_stats}
 %   \vskip 0.15in
\centering
\adjustbox{width=\linewidth}{
    \begin{tabular}{lrrrrrr}
\toprule
{} &  \# Graphs &  \# Classes &  Diameter &   Nodes &    Edges &  CC \\
\midrule
DD               &      1178 &          2 &     19.81 &  284.32 &   715.66 &          0.48 \\
ENZYMES          &       600 &          6 &     10.92 &   32.63 &    62.14 &          0.45 \\
MUTAG            &       188 &          2 &      8.22 &   17.93 &    19.79 &          0.00 \\
NCI1             &      4110 &          2 &     13.33 &   29.87 &    32.30 &          0.00 \\
NCI109           &      4127 &          2 &     13.14 &   29.68 &    32.13 &          0.00 \\
PROTEINS         &      1113 &          2 &     11.62 &   39.06 &    72.82 &          0.51 \\
PTC              &       344 &          2 &      7.52 &   14.29 &    14.69 &          0.01 \\
\midrule
COLLAB           &      5000 &          3 &      1.86 &   74.49 &  2457.22 &          0.89 \\
IMDB-B     &      1000 &          2 &      1.86 &   19.77 &    96.53 &          0.95 \\
IMDB-M       &      1500 &          3 &      1.47 &   13.00 &    65.94 &          0.97 \\
REDDIT-B    &      2000 &          2 &      8.59 &  429.63 &   497.75 &          0.05 \\
REDDIT-12K &     11929 &         11 &      9.53 &  391.41 &   456.89 &          0.03 \\
REDDIT-5K  &      4999 &          5 &     10.57 &  508.52 &   594.87 &          0.03 \\
\bottomrule
\end{tabular}}
%\vspace{-10mm}
\end{table}



==> tables/ensemble.tex <==
\begin{table}[ht]
    \centering
    \caption{Mean $\pm$ standard deviation test set accuracy on biochemical and social network datasets.}
    \scalebox{1}{
        \input{tables/raw/ensemble_raw}
    }
    \label{tab:ensemble}
\end{table}


==> tables/full_comparison_old.tex <==
\begin{table}[ht]
    \centering
     \caption{Mean $\pm$ std. over 10 test sets on bio-chemical and social datasets.}
    \scalebox{0.75}{
\begin{tabular}{llllllll}
\toprule
{} &                   LEGS-RBF &                   LEGS-FCN &         LEGS-FIXED &                        GCN &                  GraphSAGE &                     GS-SVM &                   Baseline \\
\midrule
DD               &           72.58 $\pm$ 3.35 &           72.07 $\pm$ 2.37 &   69.09 $\pm$ 4.82 &           67.82 $\pm$ 3.81 &           66.37 $\pm$ 4.45 &           72.66 $\pm$ 4.94 &  \textbf{75.98 $\pm$ 2.81} \\
ENZYMES          &           36.33 $\pm$ 4.50 &  \textbf{38.50 $\pm$ 8.18} &   32.33 $\pm$ 5.04 &           31.33 $\pm$ 6.89 &           15.83 $\pm$ 9.10 &           27.33 $\pm$ 5.10 &           20.50 $\pm$ 5.99 \\
MUTAG            &           33.51 $\pm$ 4.34 &           82.98 $\pm$ 9.85 &  81.84 $\pm$ 11.24 &           79.30 $\pm$ 9.66 &          81.43 $\pm$ 11.64 &  \textbf{85.09 $\pm$ 7.44} &           79.80 $\pm$ 9.92 \\
NCI1             &  \textbf{74.26 $\pm$ 1.53} &           70.83 $\pm$ 2.65 &   71.24 $\pm$ 1.63 &           60.80 $\pm$ 4.26 &           57.54 $\pm$ 3.33 &           69.68 $\pm$ 2.38 &           56.69 $\pm$ 3.07 \\
NCI109           &  \textbf{72.47 $\pm$ 2.11} &           70.17 $\pm$ 1.46 &   69.25 $\pm$ 1.75 &           61.30 $\pm$ 2.99 &           55.15 $\pm$ 2.58 &           68.55 $\pm$ 2.06 &           57.38 $\pm$ 2.20 \\
PROTEINS         &           70.89 $\pm$ 3.91 &           71.06 $\pm$ 3.17 &   67.30 $\pm$ 2.94 &  \textbf{74.03 $\pm$ 3.20} &           71.87 $\pm$ 3.50 &           70.98 $\pm$ 2.67 &           73.22 $\pm$ 3.76 \\
PTC              &  \textbf{57.26 $\pm$ 5.54} &           56.92 $\pm$ 9.36 &   54.31 $\pm$ 6.92 &          56.34 $\pm$ 10.29 &           55.22 $\pm$ 9.13 &           56.96 $\pm$ 7.09 &           56.71 $\pm$ 5.54 \\
\midrule
COLLAB           &           75.78 $\pm$ 1.95 &           75.40 $\pm$ 1.80 &   72.94 $\pm$ 1.70 &           73.80 $\pm$ 1.73 &  \textbf{76.12 $\pm$ 1.58} &           74.54 $\pm$ 2.32 &           64.76 $\pm$ 2.63 \\
IMDB-BINARY      &           64.90 $\pm$ 3.48 &           64.50 $\pm$ 3.50 &   64.30 $\pm$ 3.68 &           47.40 $\pm$ 6.24 &           46.40 $\pm$ 4.03 &  \textbf{66.70 $\pm$ 3.53} &           47.20 $\pm$ 5.67 \\
IMDB-MULTI       &           41.93 $\pm$ 3.01 &           40.13 $\pm$ 2.77 &   41.67 $\pm$ 3.19 &           39.33 $\pm$ 3.13 &           39.73 $\pm$ 3.45 &  \textbf{42.13 $\pm$ 2.53} &           39.53 $\pm$ 3.63 \\
REDDIT-BINARY    &  \textbf{86.10 $\pm$ 2.92} &           78.15 $\pm$ 5.42 &   85.00 $\pm$ 1.93 &           81.60 $\pm$ 2.32 &           73.40 $\pm$ 4.38 &           85.15 $\pm$ 2.78 &           69.30 $\pm$ 5.08 \\
REDDIT-MULTI-12K &           38.47 $\pm$ 1.07 &           38.46 $\pm$ 1.31 &   39.74 $\pm$ 1.31 &  \textbf{42.57 $\pm$ 0.90} &           32.17 $\pm$ 2.04 &           39.79 $\pm$ 1.11 &           22.07 $\pm$ 0.98 \\
REDDIT-MULTI-5K  &           47.83 $\pm$ 2.61 &           46.97 $\pm$ 3.06 &   47.17 $\pm$ 2.93 &  \textbf{52.79 $\pm$ 2.11} &           45.71 $\pm$ 2.88 &           48.79 $\pm$ 2.95 &           36.41 $\pm$ 1.80 \\
\bottomrule
\end{tabular}
}
   
    \label{tab:ablation}
\end{table}













\begin{tabular}{llllllllllll}
\toprule
{} &                   LEGS-RBF &                   LEGS-FCN &         LEGS-FIXED &                GCN &          GraphSAGE &               GAT &                        GIN &                     GS-SVM &                   Baseline &                   GCN-LEGS &                   GCN-SORT \\
\midrule
DD               &           72.58 $\pm$ 3.35 &           72.07 $\pm$ 2.37 &   69.09 $\pm$ 4.82 &   67.82 $\pm$ 3.81 &   66.37 $\pm$ 4.45 &  68.50 $\pm$ 3.62 &           42.37 $\pm$ 4.32 &           72.66 $\pm$ 4.94 &  \textbf{75.98 $\pm$ 2.81} &           74.02 $\pm$ 2.79 &           73.34 $\pm$ 3.57 \\
ENZYMES          &           36.33 $\pm$ 4.50 &  \textbf{38.50 $\pm$ 8.18} &   32.33 $\pm$ 5.04 &   31.33 $\pm$ 6.89 &   15.83 $\pm$ 9.10 &  25.83 $\pm$ 4.73 &           36.83 $\pm$ 4.81 &           27.33 $\pm$ 5.10 &           20.50 $\pm$ 5.99 &           31.83 $\pm$ 6.78 &           35.83 $\pm$ 5.57 \\
MUTAG            &           33.51 $\pm$ 4.34 &           82.98 $\pm$ 9.85 &  81.84 $\pm$ 11.24 &   79.30 $\pm$ 9.66 &  81.43 $\pm$ 11.64 &  79.85 $\pm$ 9.44 &           83.57 $\pm$ 9.68 &  \textbf{85.09 $\pm$ 7.44} &           79.80 $\pm$ 9.92 &           82.46 $\pm$ 7.88 &           83.54 $\pm$ 9.39 \\
NCI1             &  \textbf{74.26 $\pm$ 1.53} &           70.83 $\pm$ 2.65 &   71.24 $\pm$ 1.63 &   60.80 $\pm$ 4.26 &   57.54 $\pm$ 3.33 &  62.19 $\pm$ 2.18 &           66.67 $\pm$ 2.90 &           69.68 $\pm$ 2.38 &           56.69 $\pm$ 3.07 &           70.80 $\pm$ 2.27 &           72.21 $\pm$ 2.32 \\
NCI109           &  \textbf{72.47 $\pm$ 2.11} &           70.17 $\pm$ 1.46 &   69.25 $\pm$ 1.75 &   61.30 $\pm$ 2.99 &   55.15 $\pm$ 2.58 &  61.28 $\pm$ 2.24 &           65.23 $\pm$ 1.82 &           68.55 $\pm$ 2.06 &           57.38 $\pm$ 2.20 &           68.82 $\pm$ 1.80 &           69.52 $\pm$ 1.99 \\
PROTEINS         &           70.89 $\pm$ 3.91 &           71.06 $\pm$ 3.17 &   67.30 $\pm$ 2.94 &   74.03 $\pm$ 3.20 &   71.87 $\pm$ 3.50 &  73.22 $\pm$ 3.55 &  \textbf{75.02 $\pm$ 4.55} &           70.98 $\pm$ 2.67 &           73.22 $\pm$ 3.76 &           73.94 $\pm$ 3.88 &           74.30 $\pm$ 3.41 \\
PTC              &           57.26 $\pm$ 5.54 &           56.92 $\pm$ 9.36 &   54.31 $\pm$ 6.92 &  56.34 $\pm$ 10.29 &   55.22 $\pm$ 9.13 &  55.50 $\pm$ 6.90 &           55.82 $\pm$ 8.07 &           56.96 $\pm$ 7.09 &           56.71 $\pm$ 5.54 &  \textbf{58.11 $\pm$ 6.06} &           56.64 $\pm$ 7.34 \\
COLLAB           &           75.78 $\pm$ 1.95 &           75.40 $\pm$ 1.80 &   72.94 $\pm$ 1.70 &   73.80 $\pm$ 1.73 &   76.12 $\pm$ 1.58 &  72.88 $\pm$ 2.06 &           62.98 $\pm$ 3.92 &           74.54 $\pm$ 2.32 &           64.76 $\pm$ 2.63 &  \textbf{76.60 $\pm$ 1.75} &           75.76 $\pm$ 1.83 \\
IMDB-BINARY      &           64.90 $\pm$ 3.48 &           64.50 $\pm$ 3.50 &   64.30 $\pm$ 3.68 &   47.40 $\pm$ 6.24 &   46.40 $\pm$ 4.03 &  45.50 $\pm$ 3.14 &           64.20 $\pm$ 5.77 &  \textbf{66.70 $\pm$ 3.53} &           47.20 $\pm$ 5.67 &           65.10 $\pm$ 3.75 &           65.90 $\pm$ 4.33 \\
IMDB-MULTI       &           41.93 $\pm$ 3.01 &           40.13 $\pm$ 2.77 &   41.67 $\pm$ 3.19 &   39.33 $\pm$ 3.13 &   39.73 $\pm$ 3.45 &  39.73 $\pm$ 3.61 &           38.67 $\pm$ 3.93 &  \textbf{42.13 $\pm$ 2.53} &           39.53 $\pm$ 3.63 &           39.93 $\pm$ 2.69 &           39.87 $\pm$ 2.24 \\
REDDIT-BINARY    &           86.10 $\pm$ 2.92 &           78.15 $\pm$ 5.42 &   85.00 $\pm$ 1.93 &   81.60 $\pm$ 2.32 &   73.40 $\pm$ 4.38 &  73.35 $\pm$ 2.27 &           71.40 $\pm$ 6.98 &           85.15 $\pm$ 2.78 &           69.30 $\pm$ 5.08 &           86.90 $\pm$ 1.90 &  \textbf{87.00 $\pm$ 2.36} \\
REDDIT-MULTI-12K &           38.47 $\pm$ 1.07 &           38.46 $\pm$ 1.31 &   39.74 $\pm$ 1.31 &   42.57 $\pm$ 0.90 &   32.17 $\pm$ 2.04 &  32.74 $\pm$ 0.75 &           24.45 $\pm$ 5.52 &           39.79 $\pm$ 1.11 &           22.07 $\pm$ 0.98 &           45.41 $\pm$ 1.24 &  \textbf{45.55 $\pm$ 1.00} \\
REDDIT-MULTI-5K  &           47.83 $\pm$ 2.61 &           46.97 $\pm$ 3.06 &   47.17 $\pm$ 2.93 &   52.79 $\pm$ 2.11 &   45.71 $\pm$ 2.88 &  44.03 $\pm$ 2.57 &           35.73 $\pm$ 8.35 &           48.79 $\pm$ 2.95 &           36.41 $\pm$ 1.80 &  \textbf{53.87 $\pm$ 2.75} &           53.41 $\pm$ 3.07 \\
\bottomrule
\end{tabular}

==> tables/qm9_split.tex <==
\begin{table}[ht]
    \centering
    \caption{Mean $\pm$ std.\ over four runs of mean squared error over 19 targets for the QM9 dataset, lower is better.}
    \scalebox{0.8}{
        \input{tables/raw/qm9_split_raw}
    }
    \label{tab:qm9_split}
\end{table}


==> tables/raw/biochen_comparison_raw.tex <==
\begin{tabular}{llllllll}
\toprule
{} &                         DD &                    ENZYMES &                      MUTAG &                       NCI1 &                     NCI109 &                   PROTEINS &                        PTC \\
\midrule
LEGS-RBF   &           72.58 $\pm$ 3.35 &           36.33 $\pm$ 4.50 &           33.51 $\pm$ 4.34 &  \textbf{74.26 $\pm$ 1.53} &  \textbf{72.47 $\pm$ 2.11} &           70.89 $\pm$ 3.91 &  \textbf{57.26 $\pm$ 5.54} \\
LEGS-FCN   &           72.07 $\pm$ 2.37 &  \textbf{38.50 $\pm$ 8.18} &           82.98 $\pm$ 9.85 &           70.83 $\pm$ 2.65 &           70.17 $\pm$ 1.46 &           71.06 $\pm$ 3.17 &           56.92 $\pm$ 9.36 \\
LEGS-FIXED &           69.09 $\pm$ 4.82 &           32.33 $\pm$ 5.04 &          81.84 $\pm$ 11.24 &           71.24 $\pm$ 1.63 &           69.25 $\pm$ 1.75 &           67.30 $\pm$ 2.94 &           54.31 $\pm$ 6.92 \\
GCN        &           67.82 $\pm$ 3.81 &           31.33 $\pm$ 6.89 &           79.30 $\pm$ 9.66 &           60.80 $\pm$ 4.26 &           61.30 $\pm$ 2.99 &           74.03 $\pm$ 3.20 &          56.34 $\pm$ 10.29 \\
GraphSAGE  &           66.37 $\pm$ 4.45 &           15.83 $\pm$ 9.10 &          81.43 $\pm$ 11.64 &           57.54 $\pm$ 3.33 &           55.15 $\pm$ 2.58 &           71.87 $\pm$ 3.50 &           55.22 $\pm$ 9.13 \\
GAT        &           68.50 $\pm$ 3.62 &           25.83 $\pm$ 4.73 &           79.85 $\pm$ 9.44 &           62.19 $\pm$ 2.18 &           61.28 $\pm$ 2.24 &           73.22 $\pm$ 3.55 &           55.50 $\pm$ 6.90 \\
GIN        &           42.37 $\pm$ 4.32 &           36.83 $\pm$ 4.81 &           83.57 $\pm$ 9.68 &           66.67 $\pm$ 2.90 &           65.23 $\pm$ 1.82 &  \textbf{75.02 $\pm$ 4.55} &           55.82 $\pm$ 8.07 \\
Snowball   &           TLE &           18.00 $\pm$ 1.89 &           50.56 $\pm$ 20.87 &           48.56 $\pm$ 2.92 &           50.86 $\pm$ 2.65 &           39.36 $\pm$ 4.29 &           50.84 $\pm$ 9.32 \\
GS-SVM     &           72.66 $\pm$ 4.94 &           27.33 $\pm$ 5.10 &  \textbf{85.09 $\pm$ 7.44} &           69.68 $\pm$ 2.38 &           68.55 $\pm$ 2.06 &           70.98 $\pm$ 2.67 &           56.96 $\pm$ 7.09 \\
Baseline   &  \textbf{75.98 $\pm$ 2.81} &           20.50 $\pm$ 5.99 &           79.80 $\pm$ 9.92 &           56.69 $\pm$ 3.07 &           57.38 $\pm$ 2.20 &           73.22 $\pm$ 3.76 &           56.71 $\pm$ 5.54 \\
\bottomrule
\end{tabular}

==> tables/raw/ensemble_raw.tex <==
\begin{tabular}{llll}
\toprule
{} &                GCN &                   GCN-LEGS-FIXED &                   GCN-LEGS-FCN \\
\midrule
DD               &   67.82 $\pm$ 3.81 &  \textbf{74.02 $\pm$ 2.79} &           73.34 $\pm$ 3.57 \\
ENZYMES          &   31.33 $\pm$ 6.89 &           31.83 $\pm$ 6.78 &  \textbf{35.83 $\pm$ 5.57} \\
MUTAG            &   79.30 $\pm$ 9.66 &           82.46 $\pm$ 7.88 &  \textbf{83.54 $\pm$ 9.39} \\
NCI1             &   60.80 $\pm$ 4.26 &           70.80 $\pm$ 2.27 &  \textbf{72.21 $\pm$ 2.32} \\
NCI109           &   61.30 $\pm$ 2.99 &           68.82 $\pm$ 1.80 &  \textbf{69.52 $\pm$ 1.99} \\
PROTEINS         &   74.03 $\pm$ 3.20 &           73.94 $\pm$ 3.88 &  \textbf{74.30 $\pm$ 3.41} \\
PTC              &  56.34 $\pm$ 10.29 &  \textbf{58.11 $\pm$ 6.06} &           56.64 $\pm$ 7.34 \\
COLLAB           &   73.80 $\pm$ 1.73 &  \textbf{76.60 $\pm$ 1.75} &           75.76 $\pm$ 1.83 \\
IMDB-BINARY      &   47.40 $\pm$ 6.24 &           65.10 $\pm$ 3.75 &  \textbf{65.90 $\pm$ 4.33} \\
IMDB-MULTI       &   39.33 $\pm$ 3.13 &  \textbf{39.93 $\pm$ 2.69} &           39.87 $\pm$ 2.24 \\
REDDIT-BINARY    &   81.60 $\pm$ 2.32 &           86.90 $\pm$ 1.90 &  \textbf{87.00 $\pm$ 2.36} \\
REDDIT-MULTI-12K &   42.57 $\pm$ 0.90 &           45.41 $\pm$ 1.24 &  \textbf{45.55 $\pm$ 1.00} \\
REDDIT-MULTI-5K  &   52.79 $\pm$ 2.11 &  \textbf{53.87 $\pm$ 2.75} &           53.41 $\pm$ 3.07 \\
\bottomrule
\end{tabular}

==> tables/raw/qm9_split_raw.tex <==
\begin{tabular}{lllllll}
\toprule
{} &                    LEGS-FCN &                  LEGS-FIXED &                GCN &          GraphSAGE &                         GIN &           Baseline \\
\midrule
Target 0  &  \textbf{0.749 $\pm$ 0.025} &           0.761 $\pm$ 0.026 &  0.776 $\pm$ 0.021 &  0.876 $\pm$ 0.083 &           0.786 $\pm$ 0.032 &  0.985 $\pm$ 0.020 \\
Target 1  &  \textbf{0.158 $\pm$ 0.014} &           0.164 $\pm$ 0.024 &  0.448 $\pm$ 0.007 &  0.555 $\pm$ 0.295 &           0.191 $\pm$ 0.060 &  0.593 $\pm$ 0.013 \\
Target 2  &  \textbf{0.830 $\pm$ 0.016} &           0.856 $\pm$ 0.026 &  0.899 $\pm$ 0.051 &  0.961 $\pm$ 0.057 &           0.903 $\pm$ 0.033 &  0.982 $\pm$ 0.027 \\
Target 3  &           0.511 $\pm$ 0.012 &  \textbf{0.508 $\pm$ 0.005} &  0.549 $\pm$ 0.010 &  0.688 $\pm$ 0.216 &           0.555 $\pm$ 0.006 &  0.805 $\pm$ 0.025 \\
Target 4  &  \textbf{0.587 $\pm$ 0.007} &  \textbf{0.587 $\pm$ 0.006} &  0.609 $\pm$ 0.009 &  0.755 $\pm$ 0.177 &           0.613 $\pm$ 0.013 &  0.792 $\pm$ 0.010 \\
Target 5  &  \textbf{0.646 $\pm$ 0.013} &           0.674 $\pm$ 0.047 &  0.889 $\pm$ 0.014 &  0.882 $\pm$ 0.118 &           0.699 $\pm$ 0.033 &  0.833 $\pm$ 0.026 \\
Target 6  &           0.018 $\pm$ 0.012 &           0.020 $\pm$ 0.011 &  0.099 $\pm$ 0.011 &  0.321 $\pm$ 0.454 &  \textbf{0.012 $\pm$ 0.006} &  0.468 $\pm$ 0.005 \\
Target 7  &           0.017 $\pm$ 0.005 &           0.024 $\pm$ 0.008 &  0.368 $\pm$ 0.015 &  0.532 $\pm$ 0.405 &  \textbf{0.015 $\pm$ 0.005} &  0.379 $\pm$ 0.013 \\
Target 8  &           0.017 $\pm$ 0.005 &           0.024 $\pm$ 0.008 &  0.368 $\pm$ 0.015 &  0.532 $\pm$ 0.404 &  \textbf{0.015 $\pm$ 0.005} &  0.378 $\pm$ 0.013 \\
Target 9  &           0.017 $\pm$ 0.005 &           0.024 $\pm$ 0.008 &  0.368 $\pm$ 0.015 &  0.532 $\pm$ 0.404 &  \textbf{0.015 $\pm$ 0.005} &  0.378 $\pm$ 0.013 \\
Target 10 &           0.017 $\pm$ 0.005 &           0.024 $\pm$ 0.008 &  0.368 $\pm$ 0.015 &  0.533 $\pm$ 0.404 &  \textbf{0.015 $\pm$ 0.005} &  0.380 $\pm$ 0.014 \\
Target 11 &  \textbf{0.254 $\pm$ 0.013} &           0.279 $\pm$ 0.023 &  0.548 $\pm$ 0.023 &  0.617 $\pm$ 0.282 &           0.294 $\pm$ 0.003 &  0.631 $\pm$ 0.013 \\
Target 12 &           0.034 $\pm$ 0.014 &           0.033 $\pm$ 0.010 &  0.215 $\pm$ 0.009 &  0.356 $\pm$ 0.437 &  \textbf{0.020 $\pm$ 0.002} &  0.478 $\pm$ 0.014 \\
Target 13 &           0.033 $\pm$ 0.014 &           0.033 $\pm$ 0.010 &  0.214 $\pm$ 0.009 &  0.356 $\pm$ 0.438 &  \textbf{0.020 $\pm$ 0.002} &  0.478 $\pm$ 0.014 \\
Target 14 &           0.033 $\pm$ 0.014 &           0.033 $\pm$ 0.010 &  0.213 $\pm$ 0.009 &  0.355 $\pm$ 0.438 &  \textbf{0.020 $\pm$ 0.002} &  0.478 $\pm$ 0.014 \\
Target 15 &           0.036 $\pm$ 0.014 &           0.036 $\pm$ 0.011 &  0.219 $\pm$ 0.009 &  0.359 $\pm$ 0.436 &  \textbf{0.023 $\pm$ 0.002} &  0.479 $\pm$ 0.014 \\
Target 16 &           0.002 $\pm$ 0.002 &           0.001 $\pm$ 0.001 &  0.017 $\pm$ 0.034 &  0.012 $\pm$ 0.022 &  \textbf{0.000 $\pm$ 0.000} &  0.033 $\pm$ 0.013 \\
Target 17 &           0.083 $\pm$ 0.047 &  \textbf{0.079 $\pm$ 0.033} &  0.280 $\pm$ 0.354 &  0.264 $\pm$ 0.347 &           0.169 $\pm$ 0.206 &  0.205 $\pm$ 0.220 \\
Target 18 &  \textbf{0.062 $\pm$ 0.005} &           0.176 $\pm$ 0.231 &  0.482 $\pm$ 0.753 &  0.470 $\pm$ 0.740 &           0.321 $\pm$ 0.507 &  0.368 $\pm$ 0.525 \\
\bottomrule
\end{tabular}

==> tables/training_reduction_table.tex <==
\begin{table}[ht]
    \centering
    \caption{Mean $\pm$ std. over test set selection on cross-validated LEGS-RBF Net with reduced training set size.}
\begin{tabular}{lllll}
\toprule
Train, Val, Test \% &  80\%, 10\%, 10\% &  70\%, 10\%, 20\% &  40\%, 10\%, 50\% &  20\%, 10\%, 70\% \\
%                &                   &                   &                   &                   \\
\midrule
COLLAB           &  75.78 $\pm$ 1.95 &  75.00 $\pm$ 1.83 &  74.00 $\pm$ 0.51 &  72.73 $\pm$ 0.59 \\
DD               &  72.58 $\pm$ 3.35 &  70.88 $\pm$ 2.83 &  69.95 $\pm$ 1.85 &  69.43 $\pm$ 1.24 \\
ENZYMES          &  36.33 $\pm$ 4.50 &  34.17 $\pm$ 3.77 &  29.83 $\pm$ 3.54 &  23.98 $\pm$ 3.32 \\
IMDB-BINARY      &  64.90 $\pm$ 3.48 &  63.00 $\pm$ 2.03 &  63.30 $\pm$ 1.27 &  57.67 $\pm$ 6.04 \\
IMDB-MULTI       &  41.93 $\pm$ 3.01 &  40.80 $\pm$ 1.79 &  41.80 $\pm$ 1.23 &  36.83 $\pm$ 3.31 \\
MUTAG            &  33.51 $\pm$ 4.34 &  33.51 $\pm$ 1.14 &  33.52 $\pm$ 1.26 &  33.51 $\pm$ 0.77 \\
NCI1             &  74.26 $\pm$ 1.53 &  74.38 $\pm$ 1.38 &  72.07 $\pm$ 0.28 &  70.30 $\pm$ 0.72 \\
NCI109           &  72.47 $\pm$ 2.11 &  72.21 $\pm$ 0.92 &  70.44 $\pm$ 0.78 &  68.46 $\pm$ 0.96 \\
PROTIENS         &  70.89 $\pm$ 3.91 &  69.27 $\pm$ 1.95 &  69.72 $\pm$ 0.27 &  68.96 $\pm$ 1.63 \\
PTC              &  57.26 $\pm$ 5.54 &  57.83 $\pm$ 4.39 &  54.62 $\pm$ 3.21 &  55.45 $\pm$ 2.35 \\
REDDIT-BINARY    &  86.10 $\pm$ 2.92 &  86.05 $\pm$ 2.51 &  85.15 $\pm$ 1.77 &  83.71 $\pm$ 0.97 \\
REDDIT-MULTI-12K &  38.47 $\pm$ 1.07 &  38.60 $\pm$ 0.52 &  37.55 $\pm$ 0.05 &  36.65 $\pm$ 0.50 \\
REDDIT-MULTI-5K  &  47.83 $\pm$ 2.61 &  47.81 $\pm$ 1.32 &  46.73 $\pm$ 1.46 &  44.59 $\pm$ 1.02 \\
\bottomrule
\end{tabular}
    
    \label{tab:training_reduction}
\end{table}

